Shaping circuit for improving linearity, bandwidth, and dynamic range in ToT-based detectors

The quantitative measurement of energy deposits in particle detectors, particularly in calorimeters, is usually accomplished with the help of Analog-to-Digital converters (ADCs) due to their precision, wide measurement range, and good linearity. However, drawbacks such as power consumption, data volume, and bandwidth limit their use in the next generation of high-energy physics experiments. Time-over-threshold (ToT) systems offer simplicity, low power consumption, easy integrability, and wide bandwidth, but they lack precision, linearity, and dynamic range. In this work, we propose a shaper circuit that improves the weaknesses of ToT systems without sacrificing performance. We simulated and implemented the concept in the readout system of the Ring Imaging Cherenkov detector of the Compressed Baryonic Matter experiment at FAIR.

==> comments_CP.tex <==
Abstract:
The quantitative measurement of energy deposit in particle detectors, in particular in calorimeters, is usuallyaccomplished with help of Analog-to-Digital converters (ADC) due to...

Drawbacks such as data volume...: This is only true for Sampling ADCs. In particular in the past, often integrating ADCs (or QDCs) or peak-sensing ADCs  were used, which give a single value per measurement.

In this work, we propose ... (singular)

1) Introduction:
(visible) photons are usually not produced by nuclear interactions. Usually they come from ionization. Or Cherenkov. Or scintillation and fluorescence.
Bremsstrahlung is MeV photons. Thats not measured in a PMT.

page 2:
=======
"... it knocks out a primary electron due to the photo effect (or photo-electric effect)"-

In both SiPMs and PMTs, the output CURRENT signal: The native signal is a charge pulse. Current and voltage amplitude depend on how the sensor is terminated.

Information about the physical interaction within the detector, in particular deposited energy, can be obtained by measuring the light yield, using the fact that in both SiPMs and PMTs the signal amplification is - in good approximation - linear over a large dynamic range, and the electrical output signal (or charge) scales with the number of photons being detected.

Most particle detector readouts use some kind of Analog-to-Digital converters to quantize the output signal charge o norder to pbtain a measure of the deposited energy.

Again: There is not only sampling ADCs, but also integrating ADCs (i.e. QDCs) or peak-sensing ADCs, where sampling frequency and buffer sizes are not much of an issue ! 

"...measure the time difference between the leading- and trailing edge of the signal (usually the logic signal output of a discriminator)"

"There are different approaches for implementing analog signal discrimination required for ToT measurement: Comparing the detector pulse signal with a constant threshold, comparing with a dynamic threshold, or holding the maximum pulse amplitude"...

"have drawbacks, such as complexity in implementation, power consumption per channel"...


page 3:
=======
Figure 1 caption: "Different approaches for time-over-threshold measurement: ToT based on constant...."

In this work, we propose a simple method of signal shaping for improved ToT determination featuring good linearity, large bandwidth, ..."


page 4:
=======
"... the ToT becomes saturated as the signal amplitude (or charge) increases well above the detection threshold, ..."

"by a shaping circuit composed of a high-bandwidth Shotky-type diode (D)... as shown in Fig 2.
The basic idea utilizes the fact, that for Shottky-Diodes the reversed-bias current can be fairly large and is approximately constant over a wide range of reverse-bias voltage. When the photosensor...   ... slowly discharging the capacitor with an approximately constant current. ".
Then you can skip the next sentence "The diode works..."

Figure 2: Caption is quite brief, maybe extend a bit.
And i would stick to the standard, international sysmbol for (Shottky) diodes.

page 5:
=======
V_T (thermal voltage) (or eta*V_th) is not defined. Maybe add one sentence what is ment by "thermal voltage"...

formulas: "with the solution:"
"where" (skip commata behind)


page 6:
=======
The numbers example is somehow not plausible, and not helping to understand the circuit:
If the discharge time is 50ns with additional resistor, and 80000 ns without resistor, then 99.9 percent of current must be going through the resistor load. Then, the diode can not significantly change the discharge pattern from exponential to linear (as w/o capacitor)...

What exactly is I_s (31.7 mA) in your example ? Is this the constant reverse current through the diode, I_D in your figure 4 ?
Then the calculation is wrong: t=1 nF * (5V - 2.5V) / 31.7 mA = 80 ns ! not 80 mus !!!
For Vc=2.5 V, and R=50 Ohm, the peak current through R is I=2.5V/50Ohm=50 mA. So then it would be in the same ballpark as the diode current. That would make much more sense !!!

2.4 Temperature dependency:
===========================
I would add one introductory sentence on why looking at temp dependence here:
"What has to be taken into account in this simple circuit implementation is the potential temperatuere dependence of the diode reverses-bias current: The diode satuation current..."

And at the end of this discussion on temperature dependency, we need some some conclusion:
How big is the discharge time temp dependency in the end ? Maybe we can give some typical numbers here ?
Does this mean, the circuit needs precise temperature control of D ?
A change is diode reverse current would directly effect the ToT, and thus the charge-to-ToT calibration curve.
If we sell this approach for accurate energy measurement in calorimeters (as you write in the beginning) this is a very rucial point which needs some more discussion !

page 7:
=======

Spice simulation:''
"We add a constant bias signal offset of V_DCoffset = 2.5 V" - actually: why ? We should add some explanation here.
Maybe: ("in order to forward-bias the diode to accomodate small signal amplitudes, smaller than V_D (typical VD=?? 0.2 V for a Shottky diode ?)

"The output of the comparator is a square logic pulse "


page 8:
=======
Figure 2: "The DC-bias of the photosensor signal Vp is V_DC=2.5 V. The capacitor C_d decouples the DC offset prior to
signal discrimination."

What did you use for R ?  R=50 Ohm ??? Then the quiescent current would be quite large, 50 mA per channel ! 125 mW per channel !
Or is it 1kOhm ? Would make more sense to me, but that on eshould explain why we mentioned 50 Ohm in the example on page 6.

page 9:
=======
"... the curve thends to saturate as the amplitude increases"
"The small junction capacitance of... suppresses the low-frequency components of the shaped signal..."


page 10:
========
"The ToT resolution improves by decreasing the capacitance": really ? Where do i see this ? in figure 10 ?
But is it really the relative ToT resolution, which is improving ? Or is it just the absolute width of the band ?
If the dynamic ToT range only covers 40 instead of 140 ns, also the slope gets flatter.
The band should be >3 sharper to obtain the same charge resolution in the end.
In the text you should specify if you refere to relative or absolute resoluition.
If it is really the relative resolution which improves, that would be kind of counter intuitive to me.
Maybe one can add a picture then to undermine this statement ?


"Any improvement in ToT resolution directly promotes charge/amplitiude resolution, and further leads to improved energy resolution e.g. in a calorimeter.

chapter 4:
I would change the chapter title here:
"Circuit characterization based on measurements" or "Prototype circuit characterization"

I would add 1-2 sentences, why you suddenly use a transistor instead of a diode. This is bit of a surprise here.
Something in the direction, that HF transistors provide fast and good quality diodes for low cost...
Actually, in your spice sim: Could you not add the BFU760 transistor as a third option there, to see how it compares to the diodes ?
Then one would have to add 1-2 sentences on the idea of using a transistor instead of a diode already in the SPICE chapter.


The base-emitter capacitance should not play any role here, since it is shoted anyway. Of relevance should be the base-collector capacitance.
How the base-substrate capacitance influences the behaviour is not clear (at least to me). But it would be good to state which of the numbers is the rlevant: 21 pF base-collector, or 300 pF base-substrate. Are they in parallel ???
In your diode tests, the diode with capacitance 0.1pF was not working well, The 2nd diode with 190 pF was working well. How do these numbers now compare to the capacitance of the transistor ?

"we fed the circuit with a ... signal generated using an Agilent / by a Agilent" (not "the Agilent") 

page 11:
========

Figure 9:
can on seperate the left- and right part of the circuit a bit better in the schematc ? adding a little space left of Qs ? To separate amplifier from shaping circuit ?
And i would add the scope to the schematic. Probably you used the active probe for the scope measurements in order not to add additional load in parallel to Rs ? Since Rs has significant influence on the circuit behaviour, any additional load will as well and should be included in the schematic.

"the signal traces were recorded using a R&S RTO-1044 sampling scope (2 GHz) with ative, high-impedance probe head to mininize additional cicuit load."
For first circuit evaluation, the leading- and trailing edge and corresponding ToT (assuming a constant threshold of xx mV) were evaluated offline from the stored scope traces, their correlation with the input peak amplitude is shown in Fig. 10

We evaluated three capüacitance values... (The input impedance of the scope probe (<5 pF ???) in parallel to Cs can be neglected).

What do you mean with "input shaper signal" ? the output of the shaper circuit as input to the scope ? Or the input to the complete circuit ?
Or the output of the amplifier before entering the shaper ???

"the output amplitude behind the shaper circuit is reduced to about one third of the input signal " (after the preamp ?) So you compare left- and right side of Qs here ?

You write "The ratio improves to 0.31 ns/mV... Wha is lower ToT-per-amplitude better ? I think that depends on your ToT-measuring device. The smaller the ToT range, the more accurate you have to measure ToT. But also the better is the rate capability. This is alwas an individual compromise.
I would focus here on showing/explaining the different observed correlations, but not judge what is better and what is worse.

"atenuating the input amplitude by 70 %"

page 12:
=======
"The subsequent analöysis of the circuit was performed for Cs=47 pF''
"estimated resolution of delta_ToT/ToT = 4%" ??

caption fig. 11:
"The disrimination threshold for ToT evaluation was set to 10 mV"

"the shaper circuit was also tested using real photon sensor signals from a AFBR...SiPM."
"a pico-second laser pulser LD-405 illuminated it with light pulses of few photons per pulse and correspondingly large statistical pulse-to-pulse fluctuations in photon count and corresponding signal amplitude".

page 13:
=======
"The DIRICH front-end module provides 32 individual channels of high-precision FPGA-TDC based time meaurement.
Each channel includes a discrete transistor-based fast input amplifier (gain ~30, ~4 GHz bandwidth); signal discrimination and
subsequent leading- and trailing edge time meaurement (and data readout) is implemented on the ECP5 FPGA providing timing precision
better than 20 ps (RMS).
(Its NOT a monolithic amplifier. That was tried on the PADIWA boards, with limited success..)

Figure 13:
Maybe one could add the shaper circuit and subsequent FPGA inpiut to the circuit diagram ? To visualize the modified channel, and how it was done inside the circuit ?

page 14:
When you specify Cs and Rs here, i would add the information from the input impedance of the connected FPGA IO input (therefore adding it also to the circuit diagram). This capacitance and input impedance will add to Rs and Cs..


I am not sure if the text on the baseline scan (ahort as it is here) is understandable. And i also dont think it is essential for this paper.
Maybe one can just add a sentence that adding the shaper circuit results in a certain baseline shift due to the diode bias voltage whch has to be compensated when setting the readout thresholds.

page 15:
The "threshold" ont he y-axis is a bit missleading here. It s the baseline which is shown, not the threshold. (correctly stated in the figure caption)...
in the figure, its a "broken channel", not "damaged channel".

bottom:
"However, using the modified DIRICH channel allows to distinguish bewteen the different photon count levels of the SiPM signal.

page 16:
=======
"We propose a new shaping circuit"

"potentiating"-> "favoring its implementation" ?

"The higher the shaping capacitance the worse the TOT resolution" -> see above.






















